IMAGINE: An 8-to-1b 22nm FD-SOI Compute-In-Memory CNN Accelerator With an End-to-End Analog Charge-Based 0.15-8POPS/W Macro Featuring Distribution-Aware Data Reshaping

Charge-domain compute-in-memory (CIM) SRAMs have recently become an enticing compromise between computing efficiency and accuracy to process sub-8b convolutional neural networks (CNNs) at the edge. Yet, they commonly make use of a fixed dot-product (DP) voltage swing, which leads to a loss in effective ADC bits due to data-dependent clipping or truncation effects that waste precious conversion energy and computing accuracy. To overcome this, we present IMAGINE, a workload-adaptive 1-to-8b CIM-CNN accelerator in 22nm FD-SOI. It introduces a 1152x256 end-to-end charge-based macro with a multi-bit DP based on an input-serial, weight-parallel accumulation that avoids power-hungry DACs. An adaptive swing is achieved by combining a channel-wise DP array split with a linear in-ADC implementation of analog batch-normalization (ABN), obtaining a distribution-aware data reshaping. Critical design constraints are relaxed by including the post-silicon equivalent noise within a CIM-aware CNN training framework. Measurement results showcase an 8b system-level energy efficiency of 40TOPS/W at 0.3/0.6V, with competitive accuracies on MNIST and CIFAR-10. Moreover, the peak energy and area efficiencies of the 187kB/mm2 macro respectively reach up to 0.15-8POPS/W and 2.6-154TOPS/mm2, scaling with the 8-to-1b computing precision. These results exceed previous charge-based designs by 3-to-5x while being the first work to provide linear in-memory rescaling.

==> Sections/bio.tex <==
%%%%% This is the author's bio %%%%%

% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\vspace{-2cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Img/bio/photo_AK_IEEE_grey}}]{Adrian Kneip}(Member, IEEE) received the M.Sc. degree (summa cum laude) in Electrical Engineering from the Universit\'e catholique de Louvain (UCLouvain), Louvain-la-Neuve, Belgium, in 2019. He then joined UCLouvain's Electronics Circuits and Systems (ECS) group, where he obtained the Ph.D. degree in 2024 under the supervision of Prof. D. Bol. His research interests notably include the design of ultra-low-power digital ICs, as well as analog/mixed-signal accelerators for edge-AI chips. He has a particular interest for SRAM-based in-memory computing and hardware/software co-design aspects. Recently, he has also shown a rising interest event-based computing techniques, with a focus on event-driven graph neural networks and their hardware acceleration. Dr. Kneip is the author or co-author of several research papers in IEEE conferences and journals, receiving the Best Student Paper Award for the 2022's ESSCIRC-ESSDERC conference. He also serves as reviewer for various IEEE SSCS and CAS journals, wherein IEEE ESSCERC, ISCAS, JSSC and TCAS-I/-II. He also was Student Representative to the IEEE Benelux Section from 2020 to 2023.
\end{IEEEbiography}

\vspace{-1.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Img/bio/photo_ML_IEEE_grey}}]{Martin Lefebvre} (Member, IEEE) received the M.Sc. and Ph.D. degrees in engineering sciences from the Universit\'e catholique de Louvain (UCLouvain), Belgium, in 2017 and 2024. He is currently a post-doctoral researcher with the cognitive sensor nodes and systems (CogSys) laboratory led by Prof. C. Frenkel at Delft University of Technology (TU Delft), The Netherlands, working on neuromorphic hardware/software co-design for efficient on-chip learning. His research interests include hardware-aware machine learning algorithms, mixed-signal vision chips for embedded image processing, and low-power current reference architectures. Dr. Lefebvre serves as a reviewer for various IEEE journals and conferences including \sc{IEEE Journal of Solid-State Circuits} and \sc{IEEE Transactions on Circuits and Systems I and II}..
\end{IEEEbiography}

\vspace{-1.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Img/bio/photo_PM_IEEE_grey}}]{Pol Maistriaux} (Graduate Student Member, IEEE) (Student Member, IEEE) received the M.Sc. degree in electrical engineering from the Université catholique de Louvain (UCLouvain), Louvain-la-Neuve, Belgium, in 2021, where he is currently pursuing the Ph.D. degree with the Electronics Circuits and Systems Group, under the supervision of Prof. D. Bol. His current research interests include digital IC design and ultra-low-power receivers to enable large-scale mesh sensor networks for environmental monitoring applications.
\end{IEEEbiography}

\vspace{-1cm}

%\newpage
%\vspace{-10cm}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Img/bio/DB_2017_BW.png}}]{David Bol} (Senior Member, IEEE) received the M.Sc. degree in Electromechanical Engineering and the Ph.D degree in Engineering Science from Université catholique de Louvain (UCLouvain), Louvain-la-Neuve, Belgium in 2004 and 2008, respectively. In 2005, he was a visiting Ph.D student at the CNM National Centre for Microelectronics, Sevilla, Spain, in advanced logic design. In 2009, he was a postdoctoral researcher at intoPIX, Louvain-la-Neuve, Belgium, in low-power design for JPEG2000 image processing. In 2010, he was a visiting postdoctoral researcher at the UC Berkeley Laboratory for Manufacturing and Sustainability, Berkeley, CA, in life-cycle assessment of the semiconductor environmental impact. He is now an Associate Professor at UCLouvain. In 2015, he participated to the creation of e-peas semiconductors, Louvain-la-Neuve, Belgium.
Prof. Bol leads the Electronic Circuits and Systems (ECS) group focused on ultra-low-power design of integrated circuits for the IoT and biomedical applications including computing, power management, sensing and wireless communications. He is engaged in a social-ecological transition in the field of ICT research. He co-teaches four M.S. courses in Electrical Engineering at UCLouvain on digital, analog and mixed-signal integrated circuits and systems as well as sensors, with two B.S. courses including the course on Sustainable Development and Transition.
Prof. Bol has authored or co-authored more than 150 technical papers and conference contributions and holds three delivered patents. He (co-)received three Best Paper/Poster/Design Awards in IEEE conferences (ICCD 2008, SOI Conf. 2008, FTFC 2014). He serves as a reviewer for various journals and conferences such as IEEE JSSC, TVLSI, TCAS-I/-II. Since 2008, he presented several invited papers and keynote tutorials in international conferences including a forum presentation at IEEE ISSCC 2018.
On the private side, he pioneered the parental leave for male professors in his faculty to spend time connecting to nature with his family. 
\end{IEEEbiography}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}

